SDQ: Sparse Decomposed Quantization for LLM Inference

Recently, large language models (LLMs) have shown surprising performance in task-specific workloads as well as general tasks with the given prompts. However, to achieve unprecedented performance, recent LLMs use billions to trillions of parameters, which hinder the wide adaptation of those models due to their extremely large compute and memory requirements. To resolve the issue, various model compression methods are being actively investigated. In this work, we propose SDQ (Sparse Decomposed Quantization) to exploit both structured sparsity and quantization to achieve both high compute and memory efficiency. From our evaluations, we observe that SDQ can achieve 4x effective compute throughput with <1% quality drop.

==> mlsys2024style/sections/dummy.tex <==
\begin{table*}
    \centering          
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline 
 \textbf{OPT}   & 125M   & 350M   & 1.3B  & 2.7B  & 6.7B  & 13B   & 30B \\ \hline\hline
 Dense-WA16   &  27.65 &  22.00 & 14.62 & 12.47 & 10.86 & 10.13 & 9.56   \\ \hline % Validated with sparsegpt paper
 S-RTN-W4     &   -     & -       &   -    &  -     & 12.10 & 11.32 & 10.97     \\ \hline 
 S-GPTQ-W4    &   -    &  -      &   -    &    -   & 11.39 & 10.31 & 9.63     \\ \hline 
 S-SpQR-W4    &   -   &   -     &   -    &      - & 11.04 & 10.28 & 9.54     \\ \hline 
 \hline %2X Speed up
 S-SparseGPT-4:8&  43.99 & 38.92  &20.06  &15.04  &  12.57     &  11.83     & 10.31   \\ \hline 
 S-Wanda-4:8    & 53.12  & 58.90  & 22.21 & 16.77  &  13.55     & 13.35      &  10.87   \\ \hline 
 Q-VSQuant-WAi8b  & 27.77  & 22.01  & 14.75 & 12.50  & 10.95 & 10.14          &  9.57  \\ \hline
 Q-VSQuant-WAf8b  & 27.78  & 22.05  & 14.75 & 12.51 & 10.95      & 10.13      &  9.58   \\ \hline 
 \hline % 3.2X Speed up
 %SDQ-7:8-2:8o8b-5:8i4b           &   &   &  &  &       &       &    \\ \hline 
%alc1/8 + 3/16
%1/8 + 3/16
 SDQ-8:8-2:8o8b-6:8i4b &   & 22.43 &  &  &       &       &    \\ \hline 
 SDQ-4:4-1:4o8b-3:4i4b &   & 22.62  &  &  &       &       &    \\ \hline 
 \hline % 4X Speedup
 S-Wanda-2:8    &  1584.81& 2847.39  & 1217.73 &  6204.19 & 1028.50      & 2010.05      & 9997.60   \\ \hline 
 S-SparseGPT-2:8&  849.99      & 645.33     & 990.81 & 150.09&  189.00     & 265.05      & 97.92     \\ \hline 
 Q-VSQuant-WAi4b  & 33.10  & 28.25  & 17.84 & 14.63  & 12.02 & 11.72          &  10.61  \\ \hline 
 Q-VSQuant-WAf4b  & 30.50  & 24.31  & 16.00 & 13.29 & 11.32      & 10.57      &  9.90   \\ \hline 
 
 SDQ-W3:4-1:4o8b-2:4i4b           &        & 26.76  &  &  &       &       &    \\ \hline 
 SDQ-W7:8-1:8o8b-6:8i4b           & 29.30       & \textbf{23.02} & \textbf{15.44}  & 12.70  & \textbf{10.89 }     &\textbf{10.21}       &    \\ \hline 
 SDQ-W6:8-2:8o8b-4:8i4b            & 30.15      & 24.48   & 15.71 &\textbf{12.68}  & 10.91      & 10.27      &    \\ \hline\hline

 %SDQ-6:8-1:8o8b-5:8i4b            &       & 25.02   & &  &       &       &    \\ \hline\hline
 %SDQ-6:8-2:4i4b-2:8o8b            &       & 25.02   & &  &       &       &    \\ \hline\hline

    \end{tabular}
    \caption{Perplexity results of OPT, LLAMA-v1, LLAMA-v2 on raw-WikiText2 with various sparsification, quantization, and SDQ configurations.
    % group them by peak speed up
    % iso accuracy 
    % add spqr numbers
    }
    \label{tab:my_label}
\end{table*}
\begin{table*}
    \centering          
    \begin{minipage}{.4\textwidth}

    \begin{tabular}{|c|c|c|c|} \hline 
 %SDQ-6:8-1:8o8b-5:8i4b            &       & 25.02   & &  &       &       &    \\ \hline\hline
 %SDQ-6:8-2:4i4b-2:8o8b            &       & 25.02   & &  &       &       &    \\ \hline\hline
 \textbf{LLAMA-v1}&  7B    & 13B    & 30B   \\ \hline\hline
 Dense-WA16     &  5.68  & 5.09   & 4.10    \\ \hline % Validated with awq paper
 
 S-RTN-W4         & 6.43   & 5.55   & 4.57   \\ \hline 
 S-GPTQ-W4        & 6.13   & 5.40   & 4.48     \\ \hline 
 S-SpQR-W4        & 5.87   & 5.22   & 4.25    \\ \hline 
\hline %2X Speed up
 S-SparseGPT-4:8  & 8.61       & 7.42     & 6.15   \\ \hline 
 S-Wanda-4:8      & 8.5660       & 7.4057    & 5.9678     \\ \hline 
 Q-VSQuant-WAi8b &        &   &     \\ \hline 
 Q-VSQuant-WAf8b &        &   &    \\ \hline 
 \hline
 SDQ-8:8-2:8o8-6:8i4  &   &   &      \\ \hline 
 SDQ-4:4-1:4o8-3:4i4           &   &   &    \\ \hline 
 \hline % 4X Speedup
 S-SparseGPT-2:8  & 151.93       & 96.30     & 58.67    \\ \hline 
 S-Wanda-2:8      & 2960.99       & 2481.10 & 1228.86    \\ \hline 
 Q-VSQuant-WAi4b &        &   &    \\ \hline 
 Q-VSQuant-WAf4b &        &   &    \\ \hline 
 SDQ-3:4-1:4o8-2:4i4           &   &   &    \\ \hline 
 SDQ-7:8-1:8o8-6:8i4           &   &   &   \\ \hline 
 SDQ-6:8-2:8o8-4:8i4            &   &   & \\ \hline
    \end{tabular}
    \end{minipage}
    %\hfill

    \begin{minipage}{.4\textwidth}
        \begin{tabular}{|c|c|c|} \hline 
 %SDQ-6:8-1:8o8b-5:8i4b            &       & 25.02   & &  &       &       &    \\ \hline\hline
 %SDQ-6:8-2:4i4b-2:8o8b            &       & 25.02   & &  &       &       &    \\ \hline\hline
 \textbf{LLAMA-v2} & 7B   & 13B\\ \hline\hline
 Dense-WA16     &  5.68  & 5.09   & 4.10  &       &          & 5.47 & 4.88   \\ \hline % Validated with awq paper
 
 S-RTN-W4         & 6.43   & 5.55   & 4.57 & &       & -      & -     \\ \hline 
 S-GPTQ-W4        & 6.13   & 5.40   & 4.48 & &       & -      & -     \\ \hline 
 S-SpQR-W4        & 5.87   & 5.22   & 4.25 & &       & -      & -     \\ \hline 
\hline %2X Speed up
 S-SparseGPT-4:8  & 8.61       & 7.42     & 6.15 &  &       & 8.43      & 6.99   \\ \hline 
 S-Wanda-4:8      & 8.5660       & 7.4057    & 5.9678 &   &       &  8.60      &  7.00    \\ \hline 
 Q-VSQuant-WAi8b &        &   &  &  &       & 5.4964      & 4.9097   \\ \hline 
 Q-VSQuant-WAf8b &        &   &  &  &       & 5.4936      & 4.9012   \\ \hline 
 \hline
 SDQ-8:8-2:8o8b-6:8i4b           &   &   &  &  &       &       &    \\ \hline 
 SDQ-4:4-1:4o8b-3:4i4b           &   &   &  &  &       &       &    \\ \hline 
 \hline % 4X Speedup
 S-SparseGPT-2:8  & 151.93       & 96.30     & 58.67  & &       & 94.63      & 81.91    \\ \hline 
 S-Wanda-2:8      & 2960.9888       & 2481.1001 & 1228.8591 &   &       & 2877.32      & 1041.9862   \\ \hline 
 Q-VSQuant-WAi4b &        &   &  &  &       & 6.5953      & 5.5583   \\ \hline 
 Q-VSQuant-WAf4b &        &   &  &  &       & 5.7551      & 5.0712   \\ \hline 
 SDQ-3:4-1:4o8b-2:4i4b           &   &   &  &  &       &       &    \\ \hline 
 SDQ-7:8-1:8o8b-6:8i4b           &   &   &  &  &       &       &    \\ \hline 
 SDQ-6:8-2:8o8b-4:8i4b            &   &   & &  &       &       &    \\ \hline
    \end{tabular}
    \end{minipage} 
    \label{tab:my_label}
\end{table*}
